Mask-based Latent Reconstruction for Reinforcement Learning

For deep reinforcement learning (RL) from pixels, learning effective state representations is crucial for achieving high performance. However, in practice, limited experience and high-dimensional inputs prevent effective representation learning. To address this, motivated by the success of mask-based modeling in other research fields, we introduce mask-based reconstruction to promote state representation learning in RL. Specifically, we propose a simple yet effective self-supervised method, Mask-based Latent Reconstruction (MLR), to predict complete state representations in the latent space from the observations with spatially and temporally masked pixels. MLR enables better use of context information when learning state representations to make them more informative, which facilitates the training of RL agents. Extensive experiments show that our MLR significantly improves the sample efficiency in RL and outperforms the state-of-the-art sample-efficient RL methods on multiple continuous and discrete control benchmarks. Our code is available at https://github.com/microsoft/Mask-based-Latent-Reconstruction.

==> Tables/ablation_action_token.tex <==
\begin{table}[t]
    \vspace{0pt}
    \footnotesize % control font size
    \centering
    \caption{Ablation study of action token. \textit{\ourname~w.o. ActTok} denotes the scheme removing action tokens in the input tokens of the predictive latent decoder. We run each models for 3 random seeds.}
    \label{table:ablate_acttok}
    \scalebox{0.92}{
        \begin{tabular}{l c c c}
            \toprule
            \textbf{Env.} & \textbf{Baseline} & \textbf{\ourname~w.o. ActTok} & \textbf{\ourname}\\ \hline
            \specialrule{0em}{1.5pt}{1pt}   % control space gap
            Fing.spin & 822 $\pm$ 146 & 843 $\pm$ 34 & \textbf{904 $\pm$ 70}\\
            Cart.swin & 782 $\pm$ 74  & \textbf{822 $\pm$ 8} & 808 $\pm$ 40\\
            Reac.easy & 557 $\pm$ 137 & 840 $\pm$ 58 & \textbf{880 $\pm$ 82} \\
            Chee.run  & 438 $\pm$ 33  & 403 $\pm$ 82  & \textbf{487 $\pm$ 9} \\
            Walk.walk & 414 $\pm$ 310 & 470 $\pm$ 217  & \textbf{616 $\pm$ 87}\\
            Ball.catc & 669 $\pm$ 310 & 818 $\pm$ 141  & \textbf{932 $\pm$ 3} \\ 
            \midrule
            Mean & 613.7 & 699.3 & \textbf{771.2} \\ 
            Median & 613.0 & 820.0 & \textbf{844.0} \\ 
            \midrule
        \end{tabular}
    }
    \vspace{-5pt}
\end{table}


==> Tables/ablation_masking_strategy.tex <==
\begin{table}[t]
    \vspace{0pt}
    \footnotesize % control font size
    \centering
    \caption{Ablation study of masking strategy on DMControl-100k benchmark. We compare three masking strategies: spatial masking (\textit{\ourname-S}), temporal masking (\textit{\ourname-T}) and spatial-temporal masking (\textit{\ourname}). The results are averaged over 5 random seeds.}
    \label{table:ablate_masking_strategy}
    \scalebox{0.92}{
        \begin{tabular}{l c c c c}
            \toprule
            \textbf{Env.} & \textbf{Baseline} & \textbf{\ourname-S} & \textbf{\ourname-T} & \textbf{\ourname} \\ \hline
            \specialrule{0em}{1.5pt}{1pt}   % control space gap
            Fing.spin & 822 $\pm$ 146 & \textbf{919 $\pm$ 55}   & 787 $\pm$ 139     & 907 $\pm$ 69\\
            Cart.swin & 782 $\pm$ 74 & 665 $\pm$ 118     & \textbf{829 $\pm$ 33}      & 791 $\pm$ 50\\
            Reac.easy & 557 $\pm$ 137 & 848 $\pm$ 82    & 745 $\pm$ 84     & \textbf{875 $\pm$ 92} \\
            Chee.run & 438 $\pm$ 33 & 449 $\pm$ 46      & 443 $\pm$ 43     & \textbf{495 $\pm$ 13} \\
            Walk.walk & 414 $\pm$ 310 & 556 $\pm$ 189   & 393 $\pm$ 202     & \textbf{597 $\pm$ 102}\\
            Ball.catch & 669 $\pm$ 310 &  927 $\pm$ 6  & 934 $\pm$ 29     & \textbf{939 $\pm$ 9} \\ 
            \midrule
            Mean & 613.7 & 727.3 & 688.5 & \textbf{767.3} \\ 
            Median & 613.0 & 756.5 & 766.0 & \textbf{833.0} \\ 
            \midrule
        \end{tabular}
    }
    % \vspace{-5pt}
\end{table}


==> Tables/ablation_targets.tex <==
\begin{table}[t]
    \vspace{0pt}
    \footnotesize % control font size
    \centering
    \caption{Ablation study of reconstruction target on DMControl-100k benchmark. We compare two reconstruction targets, original pixels (denoted as \textit{\ourname-Pixel}) and momentum projections in the latent space (\ieno, \textit{\ourname}). We run each models for 5 random seeds.}
    \label{table:ablate_targets}
    \scalebox{0.92}{
        \begin{tabular}{l c c c}
            \toprule
            \textbf{Env.} & \textbf{Baseline} & \textbf{\ourname-Pixel} & \textbf{\ourname}\\ \hline
            \specialrule{0em}{1.5pt}{1pt}   % control space gap
            Fing.spin & 822 $\pm$ 146 & 782 $\pm$ 95 & \textbf{907 $\pm$ 69}\\
            Cart.swin & 782 $\pm$ 74  & \textbf{803 $\pm$ 91} & 791 $\pm$ 50\\
            Reac.easy & 557 $\pm$ 137 & 787 $\pm$ 136 & \textbf{875 $\pm$ 92} \\
            Chee.run  & 438 $\pm$ 33  & 346 $\pm$ 84  & \textbf{495 $\pm$ 13} \\
            Walk.walk & 414 $\pm$ 310 & 490 $\pm$ 216  & \textbf{597 $\pm$ 102}\\
            Ball.catch & 669 $\pm$ 310 & 675 $\pm$ 292  & \textbf{939 $\pm$ 9} \\ 
            \midrule
            Mean & 613.7 & 647.2 & \textbf{767.3} \\ 
            Median & 613.0 & 728.5 & \textbf{833.0} \\ 
            \midrule
        \end{tabular}
    }
    % \vspace{-5pt}
\end{table}


==> Tables/dmc_comparison_for_review.tex <==
\begin{table*}[t]
    % \vspace{0pt}
    \footnotesize % control font size
    \centering
    \caption{Comparison results (mean $\pm$ std) on the DMControl-100k and DMControl-500k benchmarks. Our method augments \textit{Baseline} with the proposed \ourname~objective (denoted as \textit{\ourname}).}
    %\caption{Scores (mean and standard deviation) achieved by different methods on the DMControl after 100k environment steps (DMControl-100k) and 500k environment steps (DMControl-500k). We run our \ourname~with 10 random seeds.}
    % \caption{Results (mean $\&$ standard deviation) of different methods on the DMControl at 100k environment steps (DMControl-100k) and 500k environment steps (DMControl-500k). The result of our method is averaged over 10 random seeds.}
    \label{table:dmc_compare}
    % \vspace{-5pt}
    % \scalebox{0.72}{
    \scalebox{0.75}{
        \begin{tabular}{l c c c c c c c c c}
            \toprule
            \textbf{100k Step Scores} & \textbf{PlaNet} & \textbf{Dreamer} & \textbf{SAC+AE} & \textbf{SLAC} & \textbf{CURL} & \textbf{DrQ} & \textbf{Baseline}  & \textbf{\ourname~(Ours)}\\ \hline
            \specialrule{0em}{1.5pt}{1pt}   % control space gap
            Finger, spin & 136 $\pm$ 216  & 341 $\pm$ 70   & 740 $\pm$ 64    & 693 $\pm$ 141 & 767 $\pm$ 56  & 901 $\pm$ 104  & 853 $\pm$ 112 & \textbf{907 $\pm$ 58} \\
            Cartpole, swingup & 297 $\pm$ 39   & 326 $\pm$ 27   & 311 $\pm$ 11    & -             & 582 $\pm$ 146 &  759 $\pm$ 92 & 784 $\pm$ 63 & \textbf{806 $\pm$ 48}\\
            Reacher, easy & 20 $\pm$ 50    & 314 $\pm$ 155  & 274 $\pm$ 14    & -             & 538 $\pm$ 233  & 601 $\pm$ 213 & 593 $\pm$ 118 & \textbf{866 $\pm$ 103}\\
            Cheetah, run & 138 $\pm$ 88   & 235 $\pm$ 137  & 267 $\pm$ 24    & 319 $\pm$ 56  & 299 $\pm$ 48  & 344 $\pm$ 67 & 399 $\pm$ 80 & \textbf{482 $\pm$ 38}\\
            Walker, walk  & 224 $\pm$ 48   & 277 $\pm$ 12   & 394 $\pm$ 22    & 361 $\pm$ 73  & 403 $\pm$ 24  & 612 $\pm$ 164  & 424 $\pm$ 281 & \textbf{643 $\pm$ 114}\\
            Ball in cup, catch & 0 $\pm$ 0      & 246 $\pm$ 174  & 391 $\pm$ 82    & 512 $\pm$ 110 & 769 $\pm$ 43  & 913 $\pm$ 53 & 648 $\pm$ 287 & \textbf{933 $\pm$ 16}\\ 
            \midrule
            Mean & 135.8 & 289.8 & 396.2 & 471.3 & 559.7 & 688.3& 616.8 & \textbf{772.8} \\ 
            Median & 137.0 & 295.5 & 351.0 & 436.5 & 560.0 & 685.5 & 620.5 & \textbf{836.0} \\ 
            \midrule
            \textbf{500k Step Scores}  & & & & & & & & \\ \midrule
            Finger, spin & 561 $\pm$ 284  & 796 $\pm$ 183  & 884 $\pm$ 128   & 673 $\pm$ 92  & 926 $\pm$ 45 & 938 $\pm$ 103 & 944 $\pm$ 97 & \textbf{973 $\pm$ 31}\\
            Cartpole, swingup & 475 $\pm$ 71   & 762 $\pm$ 27   & 735 $\pm$ 63    & -             & 841 $\pm$ 45& 868 $\pm$ 10 & 871 $\pm$ 4 & \textbf{872 $\pm$ 5} \\
            Reacher, easy & 210 $\pm$ 390  & 793 $\pm$ 164  & 627 $\pm$ 58    & -             & 929 $\pm$ 44 & 942 $\pm$ 71& 943 $\pm$ 52 & \textbf{957 $\pm$ 41}\\
            Cheetah, run & 305 $\pm$ 131  & 570 $\pm$ 253  & 550 $\pm$ 34    & 640 $\pm$ 19  & 518 $\pm$ 28  & 660 $\pm$ 96  & 602 $\pm$ 67 & \textbf{674 $\pm$ 37}\\
            Walker, walk  & 351 $\pm$ 58   & 897 $\pm$ 49   & 847 $\pm$ 48    & 842 $\pm$ 51  & 902 $\pm$ 43  & 921 $\pm$ 4575 &818 $\pm$ 263& \textbf{939 $\pm$ 10}\\
            Ball in cup, catch  & 460 $\pm$ 380  & 879 $\pm$ 87   & 794 $\pm$ 58    & 852 $\pm$ 71 & 959 $\pm$ 27 & 963 $\pm$ 9 & 960 $\pm$ 10& \textbf{964 $\pm$ 14}\\ 
            \midrule
            Mean & 393.7 & 782.8 & 739.5 & 751.8 & 845.8 & 882.0 & 856.3 & \textbf{896.5} \\ 
            Median & 405.5 & 794.5 & 764.5 & 757.5 & 914.0 & 929.5 & 907.0 & \textbf{948.0} \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{-5pt}
\end{table*}


==> Tables/network_params.tex <==
\begin{table}[h]
    \vspace{0pt}
    \footnotesize % control font size
    \centering
    \caption{Number of parameters of main networks in \ourname.}
    \label{table:params}
    \scalebox{1}{
        \begin{tabular}{l c c c c}
            \toprule
            \textbf{Network} & Encoder & Predictive Latent Decoder & Projection Head & Prediction Head\\ \hline
            \specialrule{0em}{1.5pt}{1pt}   % control space gap
            \textbf{Param.}  & 4.04M & 40.8K & 10.2K & 10.2K \\
            \midrule
        \end{tabular}
    }
    % \vspace{-5pt}
\end{table}

% \begin{table}[h]
%     \vspace{0pt}
%     \footnotesize % control font size
%     \centering
%     \caption{Number of parameters of main networks in \ourname.}
%     \label{table:params}
%     \scalebox{1}{
%         \begin{tabular}{l c c c c}
%             \toprule
%             \textbf{Benchmark} & Encoder & Predictive Latent Decoder & Projection Head & Prediction Head\\ \hline
%             \specialrule{0em}{1.5pt}{1pt}   % control space gap
%             \textbf{DMControl}  & 4.04M & 40.8K & 10.2K & 10.2K \\
%             \textbf{Atari}  & 4.04M & 40.8K & 10.2K & 10.2K \\
%             \midrule
%         \end{tabular}
%     }
%     % \vspace{-5pt}
% \end{table}
